EDF: Ensemble, Distill, and Fuse for Easy Video Labeling

We present a way to rapidly bootstrap object detection on unseen videos using minimal human annotations. We accomplish this by combining two complementary sources of knowledge (one generic and the other specific) using bounding box merging and model distillation. The first (generic) knowledge source is obtained from ensembling pre-trained object detectors using a novel bounding box merging and confidence reweighting scheme. We make the observation that model distillation with data augmentation can train a specialized detector that outperforms the noisy labels it was trained on, and train a Student Network on the ensemble detections that obtains higher mAP than the ensemble itself. The second (specialized) knowledge source comes from training a detector (which we call the Supervised Labeler) on a labeled subset of the video to generate detections on the unlabeled portion. We demonstrate on two popular vehicular datasets that these techniques work to emit bounding boxes for all vehicles in the frame with higher mean average precision (mAP) than any of the reference networks used, and that the combination of ensembled and human-labeled data produces object detections that outperform either alone.

==> Makefile <==
all:
	/Library/TeX/Distributions/Programs/texbin/pdflatex paper
	/Library/TeX/Distributions/Programs/texbin/bibtex paper
	/Library/TeX/Distributions/Programs/texbin/pdflatex paper
	/Library/TeX/Distributions/Programs/texbin/pdflatex paper

arxiv:
	mkdir arxiv
	cp *.sty *.bst paper.bib arxiv
	cp -r figs arxiv
	cp -r imgs arxiv
	sed '/^\s*%/d' paper.tex > arxiv/paper.tex

clean:
	rm *.aux *.log *.out
	rm paper.pdf supp.pdf
	rm -r arxiv

